PVS Embeddings of Propositional and Quantified Modal Logic

Modal logics allow reasoning about various modes of truth: for example, what it means for something to be possibly true, or to know that something is true as opposed to merely believing it. This report describes embeddings of propositional and quantified modal logic in the PVS verification system. The resources of PVS allow this to be done in an attractive way that supports much of the standard syntax of modal logic, while providing effective automation. The report introduces and formally specifies and verifies several standard topics in modal logic such as relationships between the standard modal axioms and properties of the accessibility relation, and attributes of the Barcan Formula and its converse in both constant and varying domains.

==> mathprel.tex <==
\newenvironment{commentary}{\begin{quote}\small{\bf Commentary:}}{{\bf
End of Commentary}\normalsize\end{quote}} 
\newenvironment{proof}{{\bf Proof:}}{\noindent $\Box$\\}
\newenvironment{otherproof}{{\bf Proof:}}{}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}
\newtheorem{example}{Example}
\newtheorem{constraint}{Constraint}
\newtheorem{assumption}{Assumption}
\newenvironment{mytheorem}{\begin{theorem}\rm}{\end{theorem}}
\newcommand{\qed}[0] {\rule{1ex}{1ex} \vspace{2ex}}
\newcommand{\defdef}{\mbox{$\stackrel{\rm def}{=}$}}
\def\defn{\mathrel{\defdef}}
%\newcommand{\defn}{\mbox{$\stackrel{\rm def}{=}$}}
\newcommand{\intro}[1]{\begin{itemize}\item #1 \end{itemize}}
\newcommand{\simeqrel}[1]{\stackrel{#1}{\simeq}}
\newcommand{\eqrel}[1]{\stackrel{#1}{\approx}}
\newcommand{\simrel}[1]{\stackrel{#1}{\sim}}
\newcommand{\congrel}[1]{\stackrel{#1}{\cong}}
\newcommand{\implies}{\supset}
\def\maj{\mathop{\rm maj}}
\def\min{\mathop{\rm min}}
\def\rem{\mathop{\rm rem}}
%\def\div{\mathop{\rm div}}
\newcommand{\rmand}{\mbox{\bf \ and }}
\newcommand{\rmif}{\mbox{\bf if\ }}
\newcommand{\rmiff}{\mbox{\bf \ iff \ }}
\newcommand{\rmthen}{\mbox{\bf \ then }}
\newcommand{\rmelse}{\mbox{\bf \ else }}
\newcommand{\rmend}{\mbox{\bf end}}
\newcommand{\rmendif}{\mbox{\bf \ endif}}
\newcommand{\rmotherwise}{\mbox{\bf otherwise}}
\newcommand{\rmwith}{\mbox{\bf \ with\ }}
\newcommand{\aless}{\mathrel{\mbox{\lower.9ex\hbox{$\stackrel{\textstyle <}{\sim}$}}}}
\newcommand{\amore}{\mathrel{\mbox{\lower.9ex\hbox{$\stackrel{\textstyle >}{\sim}$}}}}
\newcommand{\seqarrow}{\mathrel{\mbox{\boldmath $\rightarrow$}}}


==> moretext.tex <==
%\topmargin 12pt
\topmargin .2in
\textwidth 5.5in
\textheight 7.75in
\oddsidemargin .65in
\evensidemargin .41in
\marginparwidth 0.85in
\marginparsep 0.2in


==> prelude.tex <==
%
% define variants of the \LaTeX macro that avoid using \sc
% for use in headings
%
\def\BigLaTeX{{\rm L\kern-.36em\raise.3ex\hbox{\smaller\smaller A}\kern-.15em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
\def\BoldLaTeX{{\bf L\kern-.36em\raise.3ex\hbox{\smaller\smaller\bf A}\kern-.15em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
%\def\labelitemi{$\bullet$}
\def\labelitemii{$\circ$}
\def\labelitemiii{$\star$}
\def\labelitemiv{$\diamond$}
\newcommand{\boxref}[1]{{\setlength{\fboxsep}{0.5mm}\small\fbox{\ref{#1}}}}
\newcommand{\tcc}{{\sc tcc}}
\newcommand{\tccs}{{\sc tcc}s}
\newcommand{\emacs}{{\sc Emacs}}
\newcommand{\Emacs}{{\sc Emacs}}
\newcommand{\ehdm}{{\sc Ehdm}}
\newcommand{\Ehdm}{{\sc Ehdm}}
\newcommand{\bigEhdm}{E{\smaller HDM}}
\newcommand{\bfehdm}{{\bf E{\smaller\bf HDM}}}
\newcommand{\itehdm}{{\it E{\smaller\it HDM}}}
\newcommand{\slehdm}{{\sl E{\smaller\sl HDM}}}
\newcommand{\murphi}{Mur$\phi$}
\newcommand{\Murphi}{Mur$\phi$}
\newcommand{\tm}{$^{\mbox{\tiny TM}}$}
\newcommand{\hozline}{{\noindent\rule{\textwidth}{0.4mm}}}
\newcommand{\allclear}{\mbox{\boldmath$\stackrel{\raisebox{-.2ex}[0pt][0pt]{$\textstyle\oslash$}}{\displaystyle\bot}$}}
\newenvironment{private}{}{}
\newenvironment{smalltt}{\begin{alltt}\small\tt}{\end{alltt}}
\newenvironment{mysmalltt}{\vspace{-1ex}\begin{alltt}\small\tt}{\end{alltt}\vspace{-1ex}}
\newenvironment{tinyalltt}{\begin{alltt}\tiny\tt}{\end{alltt}}
\newlength{\hsbw}
\newenvironment{slidesession}{\begin{flushleft}
 \setlength{\hsbw}{\linewidth}
 \addtolength{\hsbw}{-\arrayrulewidth}
 \addtolength{\hsbw}{-\tabcolsep}
 \begin{tabular}{@{}|c@{}|@{}}\hline 
 \begin{minipage}[b]{\hsbw}
 \begingroup\mbox{ }\\[-1.6\baselineskip]\begin{alltt}}{\end{alltt}\endgroup\end{minipage}\\ \hline 
 \end{tabular}
 \end{flushleft}}
\newenvironment{dslidesession}{\begin{flushleft}
 \setlength{\hsbw}{\linewidth}
 \addtolength{\hsbw}{-\arrayrulewidth}
 \addtolength{\hsbw}{-\tabcolsep}
 \begin{tabular}{@{}|c@{}|@{}}\hline 
 \begin{minipage}[b]{\hsbw}
 \begingroup\mbox{ }\\[-1.2\baselineskip]\begin{alltt}}{\end{alltt}\endgroup\end{minipage}\\ \hline 
 \end{tabular}
 \end{flushleft}}
\newenvironment{session}{\begin{flushleft}
 \setlength{\hsbw}{\linewidth}
 \addtolength{\hsbw}{-\arrayrulewidth}
 \addtolength{\hsbw}{-\tabcolsep}
 \begin{tabular}{@{}|c@{}|@{}}\hline 
 \begin{minipage}[b]{\hsbw}
% \begingroup\small\mbox{ }\\[-1.8\baselineskip]\begin{alltt}}{\end{alltt}\endgroup\end{minipage}\\ \hline
 \begingroup\sessionsize\vspace*{1.2ex}\begin{alltt}}{\end{alltt}\endgroup\end{minipage}\\ \hline
 \end{tabular}
 \end{flushleft}}
\def\extrawidth{0.5in}
\newenvironment{widesession}{\begin{flushleft}
 \setlength{\hsbw}{\linewidth}
 \addtolength{\hsbw}{\extrawidth}
 \addtolength{\hsbw}{-\arrayrulewidth}
 \addtolength{\hsbw}{-\tabcolsep}
 \begin{tabular}{@{}|c@{}|@{}}\hline 
 \begin{minipage}[b]{\hsbw}
% \begingroup\small\mbox{ }\\[-1.8\baselineskip]\begin{alltt}}{\end{alltt}\endgroup\end{minipage}\\ \hline
 \begingroup\sessionsize\vspace*{1.2ex}\begin{alltt}}{\end{alltt}\endgroup\end{minipage}\\ \hline
 \end{tabular}
 \end{flushleft}}
\def\invisiblespec{\comment}
\def\endinvisiblespec{\endcomment}
\newenvironment{sessionlab}[1]{\begin{flushleft}
 \setlength{\hsbw}{\linewidth}
 \addtolength{\hsbw}{-\arrayrulewidth}
 \addtolength{\hsbw}{-\tabcolsep}
 \begin{tabular}{@{}|c@{}|@{}}\hline 
 \begin{minipage}[b]{\hsbw}
 \vspace*{-.5pt}
 \begin{flushright}
 \rule{0.01in}{.15in}\rule{0.9in}{0.01in}\hspace{-0.95in}
 \raisebox{0.04in}{\makebox[0.9in][c]{\footnotesize #1}}
 \end{flushright}
 \vspace*{-.47in}
 \begingroup\small\vspace*{1.0ex}\begin{alltt}}{\end{alltt}\endgroup\end{minipage}\\ \hline 
 \end{tabular}
 \end{flushleft}}
\newcounter{sessioncount}
\setcounter{sessioncount}{0}
% ---------------------------------------------------------------------
% Macros for little PVS sessions displayed in boxes.
%
% Usage: (1) \setcounter{sessioncount}{1} resets the session counter
%
%	 (2) \begin{session*}\label{thissession}
%	      .
%	       < lines from PVS session >
%	      .
%	     \end{session*}
%
%            typesets the session in a numbered box in ALLTT mode.
%
%  session instead of session* produces unnumbered boxes
%
% ---------------------------------------------------------------------
\newenvironment{session*}{\begin{flushleft}
 \refstepcounter{sessioncount}
 \setlength{\hsbw}{\linewidth}
 \addtolength{\hsbw}{-\arrayrulewidth}
 \addtolength{\hsbw}{-\tabcolsep}
 \begin{tabular}{@{}|c@{}|@{}}\hline 
 \begin{minipage}[b]{\hsbw}
 \vspace*{-.5pt}
 \begin{flushright}
 \rule{0.01in}{.15in}\rule{0.3in}{0.01in}\hspace{-0.35in}
 \raisebox{0.04in}{\makebox[0.3in][c]{\footnotesize \thesessioncount}}
 \end{flushright}
 \vspace*{-.57in}
 \begingroup\small\vspace*{1.0ex}\begin{alltt}}{\end{alltt}\endgroup\end{minipage}\\ \hline 
 \end{tabular}
 \end{flushleft}}
\def\sessionsize{\small}
\def\smallsessionsize{\small}
\newenvironment{smallsession}{\begin{flushleft}
 \setlength{\hsbw}{\linewidth}
 \addtolength{\hsbw}{-\arrayrulewidth}
 \addtolength{\hsbw}{-\tabcolsep}
 \begin{tabular}{@{}|c@{}|@{}}\hline 
 \begin{minipage}[b]{\hsbw}
 \begingroup\smallsessionsize\mbox{ }\\[-1.8\baselineskip]\begin{alltt}}{\end{alltt}\endgroup\end{minipage}\\ \hline 
 \end{tabular}
 \end{flushleft}}
\newenvironment{spec}{\begin{flushleft}
 \setlength{\hsbw}{\textwidth}
 \addtolength{\hsbw}{-\arrayrulewidth}
 \addtolength{\hsbw}{-\tabcolsep}
 \begin{tabular}{@{}|c@{}|@{}}\hline 
 \begin{minipage}[b]{\hsbw}
 \begingroup\small\mbox{
}\\[-0.2\baselineskip]}{\endgroup\end{minipage}\\ \hline 
 \end{tabular}
 \end{flushleft}}
\newcommand{\exmemo}[1]{}
\newcommand{\memo}[1]{\mbox{}\par\vspace{0.25in}%
\setlength{\hsbw}{\linewidth}%
\addtolength{\hsbw}{-2\fboxsep}%
\addtolength{\hsbw}{-2\fboxrule}%
\noindent\fbox{\parbox{\hsbw}{{\bf Memo: }#1}}\vspace{0.25in}}
\newcommand{\nb}[1]{\mbox{}\par\vspace{0.25in}\setlength{\hsbw}{\linewidth}\addtolength{\hsbw}{-1.5ex}\noindent\fbox{\parbox{\hsbw}{{\bf Note: }#1}}\vspace{0.25in}}
\newcommand{\mem}[2]{\mbox{}\par\vspace{0.25in}%
\setlength{\hsbw}{\linewidth}%
\addtolength{\hsbw}{-2\fboxsep}%
\addtolength{\hsbw}{-2\fboxrule}%
\noindent\fbox{\parbox{\hsbw}{{\bf #1: }#2}}\vspace{0.25in}}
\newcommand{\comment}[1]{}
\newcommand{\excomment}[1]{#1}
%\def\comment#1{}   % Shankar doesn't like this, but the other defn
%		   % gives me errors
\newcommand{\exfootnote}[1]{}
%\newcommand{\ifelse}[2]{#1}
\sloppy
\clubpenalty=100000
\widowpenalty=100000
%\displaywidowpenalty=100000
\setcounter{secnumdepth}{3} 
\setcounter{tocdepth}{3}
\setcounter{topnumber}{9}
\setcounter{bottomnumber}{9}
\setcounter{totalnumber}{9}
\renewcommand{\topfraction}{.99}
\renewcommand{\bottomfraction}{.99}
\renewcommand{\floatpagefraction}{.01}
\renewcommand{\textfraction}{.2}
\font\largett=cmtt10 scaled\magstep1
\font\Largett=cmtt10 scaled\magstep2
\font\hugett=cmtt10 scaled\magstep3
\newcommand{\take}[1]{\\\hozline\paragraph*{From file {\tt #1}}\input{#1}\hozline}
\newlength{\sblen}
\newlength{\overhang}
%\setlength{\overhang}{0pt}
\newenvironment{sidebar}%
{\begin{figure}[htb]%
 \begin{Sbox}%
 \setlength{\sblen}{\textwidth}%
 \addtolength{\sblen}{-2\fboxsep}%
 \addtolength{\sblen}{-2\fboxrule}%
 \addtolength{\sblen}{-\overhang}%
 \begin{minipage}{\sblen}}%
{\end{minipage}\end{Sbox}\shadowbox{\TheSbox}\end{figure}}
\newenvironment{sidepage}%
{\begin{figure}[p]%
 \begin{Sbox}%
 \setlength{\sblen}{\textwidth}%
 \addtolength{\sblen}{-2\fboxsep}%
 \addtolength{\sblen}{-2\fboxrule}%
 \addtolength{\sblen}{-\overhang}%
 \begin{minipage}{\sblen}\parindent=1.5em}%
{\end{minipage}\end{Sbox}\shadowbox{\TheSbox}\end{figure}}
\def\SetFigFont#1#2#3{\rm}
\newcommand{\ul}[1]{\underline{\rule[-0.50ex]{0pt}{1ex}#1}}
\newcommand{\ttilde}{\raisebox{-.5ex}{\tt \~{}}}
\newcommand{\excite}[1]{}
%\newcommand{\hand}{$\Rightarrow$}
\newcommand{\hand}{\ ($\Rightarrow$)}
\newcommand{\nls}{\\\hspace*{1em}}
\def\srilogo{\includegraphics[height=18mm]{srilogo}}
%\newtheorem{definition}{Definition}
%\newtheorem{lemma}{Lemma}
%\newtheorem{theorem}{Theorem}
\newcommand{\etal}{\emph{et al}}
\def\widesp{0in}

